The Reversing Machine: Reconstructing Memory Assumptions

Existing anti-malware software and reverse engineering toolkits struggle with stealthy sub-OS rootkits due to limitations of run-time kernel-level monitoring. A malicious kernel-level driver can bypass OS-level anti-virus mechanisms easily. Although static analysis of such malware is possible, obfuscation and packing techniques complicate offline analysis. Moreover, current dynamic analyzers suffer from virtualization performance overhead and create detectable traces that allow modern malware to evade them. To address these issues, we present \textit{The Reversing Machine} (TRM), a new hypervisor-based memory introspection design for reverse engineering, reconstructing memory offsets, and fingerprinting evasive and obfuscated user-level and kernel-level malware. TRM proposes two novel techniques that enable efficient and transparent analysis of evasive malware: hooking a binary using suspended process creation for hypervisor-based memory introspection, and leveraging Mode-Based Execution Control (MBEC) to detect user/kernel mode transitions and memory access patterns. Unlike existing malware detection environments, TRM can extract full memory traces in user and kernel spaces and hook the entire target memory map to reconstruct arrays, structures within the operating system, and possible rootkits. We perform TRM-assisted reverse engineering of kernel-level structures and show that it can speed up manual reverse engineering by 75\% on average. We obfuscate known malware with the latest packing tools and successfully perform similarity detection. Furthermore, we demonstrate a real-world attack by deploying a modified rootkit onto a driver that bypasses state-of-the-art security auditing tools. We show that TRM can detect each threat and that, out of 24 state-of-the-art AV solutions, only TRM can detect the most advanced threats.

==> sec/AA-back.tex <==
\section{Extended Background}
\label{appen:AA}
This appendix covers additional background knowledge that did not fit the main paper

\subsection{Processor-Based VM-Execution Controls}

\subsubsection{Primary Processor-Based VM-Execution Controls}
These controls are primarily set in the VM-execution control fields, which are part of the VMCS (Virtual Machine Control Structure). The Primary Processor-Based VM-Execution Control bits enable various features and capabilities, such as interrupt handling, I/O instructions handling, and CPU feature controls, essential for managing and isolating the behavior of virtual machines.

\subsubsection{Secondary Processor-Based VM-Execution Controls }

Secondary Processor-Based VM-execution controls extend the capabilities controlled by primary processor-based controls. It is introduced in newer generations of processors, these secondary controls offer further control over CPU features in a virtualized environment. For example, they allow for enabling Extended Page Tables (EPT). Other features controlled by secondary controls include enabling Virtual Processor Identifiers (VPIDs) to reduce overhead from TLB flushes, support for unrestricted guests, and management of various other hardware-assisted virtualization features.
